HyperNAT: Scaling Up Network AddressTranslation with SmartNICs for Clouds

Network address translation (NAT) is a basic functionality in cloud gateways. With the increasing traffic volume and number of flows introduced by the cloud tenants, the NAT gateway needs to be implemented on a cluster of servers. We propose to scale up the gateway servers, which could reduce the number of servers so as to reduce the capital expense and operation expense. We design HyperNAT, which leverages smartNICs to improve the server's processing capacity. In HyperNAT, the NAT functionality is distributed on multiple NICs, and the flow space is divided and assigned accordingly. HyperNAT overcomes the challenge that the packets in two directions of one connection need to be processed by the same NAT rule (named two-direction consistency, TDC) by cloning the rule to both data paths of the two directions. Our implementation and evaluation of HyperNAT show that HyperNAT could scale up cloud gateway effectively with low overhead.

==> temp.tex <==
Network address translation (NAT) is a basic functionality in cloud gateways. With the increasing traffic volume and number of flows introduced by the cloud tenants, the NAT gateway needs to be implemented on a cluster of servers. We propose to scale up the gateway servers, which could reduce the number of servers so as to reduce the capital expense and operation expense. We design HyperNAT, which leverages smartNICs to improve the server's processing capacity. In HyperNAT, the NAT functionality is distributed on multiple NICs, and the flow space is divided and assigned accordingly. HyperNAT overcomes the challenge that the packets in two directions of one connection need to be processed by the same NAT rule (named two-direction consistency, TDC) by cloning the rule to both data paths of the two directions. Our implementation and evaluation of HyperNAT show that HyperNAT could scale up cloud gateway effectively with low overhead.

Network address translation, SmartNICs, Cloud gateway
